Speed Scaling with Multiple Servers Under A Sum Power Constraint

The problem of scheduling jobs and choosing their respective speeds with multiple servers under a sum power constraint to minimize the flow time + energy is considered. This problem is a generalization of the flow time minimization problem with multiple unit-speed servers, when jobs can be parallelized, however, with a sub-linear, concave speedup function $k^{1/\alpha}, \alpha>1$ when allocated $k$ servers, i.e., jobs experience diminishing returns from being allocated additional servers. When all jobs are available at time $0$, we show that a very simple algorithm EQUI, that processes all available jobs at the same speed is $\left(2-\frac{1}{\alpha}\right) \frac{2}{\left(1-\left(\frac{1}{\alpha}\right)\right)}$-competitive, while in the general case, when jobs arrive over time, an LCFS based algorithm is shown to have a constant (dependent only on $\alpha$) competitive ratio.

==> Equiv-ParallelSlowdown-SpeedScaling.tex <==
\section{Equivalence between the parallel scheduling model of heSRPT
  and speed scaling with net power constraint}

We use the notation from [heSRPT]: $N$ parallel and identical servers,
$M$ jobs. Size of job~$i$ is $x_i.$ Let $k_i$ denote the `number' of
servers alloted to job~$i,$ then the service rate experienced by
job~$i$ is $s_i = S(k_i) = k_i^p,$ where $p \in (0,1).$ Here,
$S(\cdot)$ denotes the speedup function. Note that
$\sum_{i = 1}^M k_i \leq N.$

Equivalently, suppose that each job has its own (solo) server, and let
$s_i$ denote the speed allocated to the server processing job~$i$
(note that each job can be allocated a non-zero speed, which makes
this an infinite server model). Interpret
$k_i = P(s_i) := S^{-1}(s_i)$ as the power consumption of job~$i.$
Note that $P(s) = s^{1/p}$ is convex increasing. Thus, the constraint
$\sum_{i=1}^M k_i \leq N$ becomes
$$\sum_{i=1}^M P(s_i) \leq N,$$ which can be thought of as a total
power constraint.

In both interpretations, the service speed of job~$i$ is $s_i,$ so the
flow times across both would be identical.

